MultiAct: Long-Term 3D Human Motion Generation from Multiple Action Labels

We tackle the problem of generating long-term 3D human motion from multiple action labels. Two main previous approaches, such as action- and motion-conditioned methods, have limitations to solve this problem. The action-conditioned methods generate a sequence of motion from a single action. Hence, it cannot generate long-term motions composed of multiple actions and transitions between actions. Meanwhile, the motion-conditioned methods generate future motions from initial motion. The generated future motions only depend on the past, so they are not controllable by the user's desired actions. We present MultiAct, the first framework to generate long-term 3D human motion from multiple action labels. MultiAct takes account of both action and motion conditions with a unified recurrent generation system. It repetitively takes the previous motion and action label; then, it generates a smooth transition and the motion of the given action. As a result, MultiAct produces realistic long-term motion controlled by the given sequence of multiple action labels. Codes are available here at https://github.com/TaeryungLee/MultiAct_RELEASE.

==> src/table1.tex <==
\begin{table}[t]
    \aboverulesep=0ex
    \belowrulesep=0ex
    % \vspace{-3mm}
    \centering
    
    \vspace{1mm}
    \setlength{\tabcolsep}{6pt}
    \resizebox{8.3cm}{!}{
        \begin{tabular}{l||cc||lc}
        \toprule
        \textbf{Notation} & \multicolumn{2}{c||}{\textbf{MACVAE (Local coordinate motions)}} & \multicolumn{2}{c}{\textbf{MultiAct (Global coordinate motions)}} \\
        
        \toprule
        \multirow{3}{*}{\textbf{Motion}} & Previous motion & $\mathscr{S}_p = \{\mathbf{p}_i\}^{l_p}_{i=1}$ & \multicolumn{1}{c}{Action motions} & $\{S_j\}^N_{j=1}$ \\
        
        & Transition & $\mathscr{T} = \{\mathbf{p}_i\}^{l_t}_{i=1}$ & \multicolumn{1}{c}{Transitions} & $\{T_j\}^N_{j=1}$ \\
        
        & Next motion & $\mathscr{S}_c = \{\mathbf{p}_i\}^{l_c}_{i=1}$ & \multicolumn{1}{c}{Long-term motions} & $\{S_1, T_2, S_2, ..., S_N\}$ \\
        
        \midrule
        \multirow{2}{*}{\textbf{Action label}} & Previous action label & $\mathfrak{a}_p \in A \subset \mathbb{Z^+}$ & \multicolumn{1}{c}{\multirow{2}{*}{Action labels}} & \multirow{2}{*}{$\{a_j  \in A \}^N_{j=1}$} \\
        
        & Next action label & $\mathfrak{a}_c \in A \subset \mathbb{Z^+}$ & \multicolumn{1}{c}{} &  \\
        
        \midrule
        \multirow{4}{*}{\textbf{Pose}} & 3D Pose & $\mathbf{p}_i = (\textbf{r}_i, \text{vec}(\theta_i), \textbf{x}_i) $ & \multicolumn{2}{l}{\multirow{4}{*}{}} \\
        & Global rotation & $\textbf{r}_i \in \mathbb{R}^6$ & \multicolumn{2}{l}{} \\
        
        & Local joint rotations & $\theta_i \in \mathbb{R}^{51\times6}$ & \multicolumn{2}{l}{} \\
        
        & Translation & $\textbf{x}_i \in \mathbb{R}^3$ & \multicolumn{2}{l}{} \\
        
        \midrule
        \multirow{2}{*}{\textbf{Length}} & Len. of $\mathscr{S}_p, \mathscr{T}, \mathscr{S}_c$ & $l_p, l_t, l_c$ & \multicolumn{2}{l}{\multirow{2}{*}{}} \\
        
        % & Len. of $\mathscr{T}$ & $l_t$ & \multicolumn{2}{l}{} \\
        
        % & Len. of $\mathscr{S}_c$ & $l_c$ & \multicolumn{2}{l}{} \\
        
        & Len. of $[\mathscr{S}_p,\ \mathscr{T},\ \mathscr{S}_c]$ & $L = l_p + l_t + l_c$ & \multicolumn{2}{l}{} \\
        \bottomrule
            
    \end{tabular}
    }
    \vspace{-1mm}
    
    \caption{
        \textbf{Notations.}
        We list important notations used in our method. 
        The first column refers to the motions in each step of MACVAE, and the second column indicate motions with multiple actions of MultiAct.
        Motions used in each step of MACVAE are \emph{canonicalized} onto the local coordinate, while the global coordinate is equivalent to the world coordinate.
        % local motion / global motion의 의미
    }
    \vspace{-6mm}
    \label{tab:table1_notation}
\end{table}
